Graph Soft-Contrastive Learning via Neighborhood Ranking

Graph Contrastive Learning (GCL) has emerged as a promising approach in the realm of graph self-supervised learning. Prevailing GCL methods mainly derive from the principles of contrastive learning in the field of computer vision: modeling invariance by specifying absolutely similar pairs. However, when applied to graph data, this paradigm encounters two significant limitations: (1) the validity of the generated views cannot be guaranteed: graph perturbation may produce invalid views against semantics and intrinsic topology of graph data; (2) specifying absolutely similar pairs in the graph views is unreliable: for abstract and non-Euclidean graph data, it is difficult for humans to decide the absolute similarity and dissimilarity intuitively. Despite the notable performance of current GCL methods, these challenges necessitate a reevaluation: Could GCL be more effectively tailored to the intrinsic properties of graphs, rather than merely adopting principles from computer vision? In response to this query, we propose a novel paradigm, Graph Soft-Contrastive Learning (GSCL). This approach facilitates GCL via neighborhood ranking, avoiding the need to specify absolutely similar pairs. GSCL leverages the underlying graph characteristic of diminishing label consistency, asserting that nodes that are closer in the graph are overall more similar than far-distant nodes. Within the GSCL framework, we introduce pairwise and listwise gated ranking InfoNCE loss functions to effectively preserve the relative similarity ranking within neighborhoods. Moreover, as the neighborhood size exponentially expands with more hops considered, we propose neighborhood sampling strategies to improve learning efficiency. Our extensive empirical results across 11 commonly used graph datasets-including 8 homophily graphs and 3 heterophily graphs-demonstrate GSCL's superior performance compared to 20 SOTA GCL methods.

==> 6-related_work.tex <==
\section{Related Work}



\subsection{Graph Representation Learning}
Graph representation learning aims to embed graphs and nodes into low-dimensional embedding spaces while preserving the attributes and structural features of graphs.
Early shallow methods such as DeepWalk \cite{perozzi2014deepwalk}, Node2vec \cite{grover2016node2vec}, and LINE \cite{tang2015line} convert graph data into a sequence of nodes by random walks, and then use language models~\cite{mikolov2013distributed} to learn the node representation.
They overemphasise the proximity of nodes at the expense of the structure of the graph~\cite{Velickovic2019DeepGI}.
G2G~\cite{bojchevski2017deep} adopts a personalized ranking formulation w.r.t. the node distances that exploits the natural ordering of the nodes imposed by the graph structure to learn the embeddings.
The ranking idea of G2G is similar to our proposed GSCL, but the ranking in G2G is to introduce graph structure information in graph Gaussian embedding, while the ranking in GSCL is to design GCL from the graph perspective to make GCL more reasonable.
Moreover, the goal of G2G is to make all closer neighbors must be more similar than all further neighbors, while GSCL describes an overall similarity ranking trend, {\it i.e.},  nodes that are closer in the graph are overall more similar than far-distant nodes.
Therefore, all the motivations, assumptions, methods, and implementations of ranking of G2G and GSCL are different.
Currently, graph neural network (GNN) methods such as GCN~\cite{welling2016semi}, GAT~\cite{Velickovic2018GraphAN}, GIN~\cite{xu2018powerful} have become the de facto standard of graph representation learning, 
they perform message passing iteratively between neighbouring nodes to capture the rich structural information in the graph.
GNN is believed to implicitly assume strong homophily~\cite{zhu2021graph, zhu2020beyond}.


\subsection{Graph Contrastive Learning}
The mainstream graph contrastive learning (GCL) is similar to the contrastive learning in computer vision. 
The first step is to generate two graph views using data augmentation. 
After that, the two graph views are fed into a shared GNN for the purpose of learning representations, which are then optimized using a contrastive learning objective function~\cite{hjelm2018learning,oord2018representation}.
Most GCL use similar graph data augmentation like topology augmentation and feature augmentation~\cite{Velickovic2019DeepGI,Zhu2020DeepGC,thakoor2021large}.
The optimal data augmentation required for different types of graph data is inconsistent, thus making data augmentation an important and sensitive hyper-parameter~\cite{you2020graph,Xia2022SimGRACEAS,Zhu2021AnES}.
To address this issue, some methods use adaptable, dynamic data augmentation for specific graph data~\cite{Zhu2020DeepGC,You2021GraphCL}.
And more recently, some methods have attempted to generate graph views without data augmentation, but instead by adding noise to the hidden embedding space~\cite{Yu2022AreGA,Zhang2022COSTACF} or model parameters~\cite{Xia2022SimGRACEAS}.
Furthermore, {\it SUGRL} feeds the same graph into a multi-layer perceptron and a GCN to generate two positive graph views~\cite{Mo2022SimpleUG}; 
{\it AFGRL} uses the original graph as one view, and generate another view by searching, for each node in the original graph, nodes that can serve as positive samples via k-nearest-neighbor (k-NN) search in the representation space~\cite{Lee2022AugmentationFreeSL}. 
Despite variations in motivations and implementations, the fundamental ideas underlying all these GCL methods are the same, {\it i.e.}, modeling invariance by specifying absolutely similar pairs.
Our proposed GSCL abandons such setting, but performs GCL in a soft and relative manner by preserving the ranking relationship of similarities in the neighborhood.  
